A Relearning Approach to Reinforcement Learning for Control of Smart Buildings

This paper demonstrates that continual relearning of control policies using incremental deep reinforcement learning (RL) can improve policy learning for non-stationary processes. We demonstrate this approach for a data-driven 'smart building environment' that we use as a test-bed for developing HVAC controllers for reducing energy consumption of large buildings on our university campus. The non-stationarity in building operations and weather patterns makes it imperative to develop control strategies that are adaptive to changing conditions. On-policy RL algorithms, such as Proximal Policy Optimization (PPO) represent an approach for addressing this non-stationarity, but exploration on the actual system is not an option for safety-critical systems. As an alternative, we develop an incremental RL technique that simultaneously reduces building energy consumption without sacrificing overall comfort. We compare the performance of our incremental RL controller to that of a static RL controller that does not implement the relearning function. The performance of the static controller diminishes significantly over time, but the relearning controller adjusts to changing conditions while ensuring comfort and optimal energy performance.

==> Sections/Preliminaries.tex <==
The environment $\mathit{E}$ has to implement the the functions $f_h,f_v,f_c$ as described in Section \ref{Reward Signal} as they will be used to calculate the energy and valve state. We use Long Short-Term Memory(\textit{LSTM}) Neural Networks to model these functions because the energy as well other data have trends in them or in other words non-stationary. Hence LSTMs are ideal candidates fr modeling such data compared to ARIMA models where non-stationarity has to be removed before the model can be fitted. 

\subsection{Long Short-Term Memory Networks}\label{LSTM}
% Marcos, can you add the LSTM from ACC paper?
\input{LSTM}

Next we shall discuss in brief the reinforcement learning algorithm that we are going to use in our problem. Proximal Policy Optimization is one of the best known reinforcement learning algorithm that can be used to learn an optimal control within a short period of time.

\subsection{Proximal Policy Optimization}\label{PPO}
\input{PPO}
